The Firewall Paradox

In this MSc. thesis, we have attempted to give an overview of the firewall paradox and various approaches towards its resolution. After an introductory chapter on some basic concepts in quantum field theory in curved spacetimes such as Hawking radiation, we introduce the paradox. It arises out of application of principles each of which is thought or assumed to be correct: 1) unitary black hole evaporation, 2) validity of quantum field theory in curved spacetime, 3) a measure of the number of black hole quantum states, 4) Einstein's equivalence principle. Then, we present various approaches that exist in the literature towards the resolution of the paradox.

==> content/apologia.tex <==
% -*- TeX-master: "\.\./thesis\.tex"; -*-

\chapter{An Apologia for Firewalls}
\label{chap:apologia}

In another article named ``An apologia for firewalls'' \cite{Almheiri2013}, with the addition of Douglas Stanford\ip{Stanford, Douglas} as the fifth author, the AMPSS defended the existence of a firewall against the critics. As Sean Carroll\ip{Carroll, Sean} mentioned in his blog-post \cite{carroll-firewall-blog} the word \emph{apologia} ``means ``defense,'' not ``apology.'' '' We briefly mention in this chapter the criticisms that are faced by various solution proposals to the paradox.


Harlow-Hayden Conjecture.


Strong Complementarity. A working model that solves the paradox needs to be shown \cite{Almheiri2013}. For example, AMPSS \cite{Almheiri2013} state that ``the most developed version'' \cite{Almheiri2013} which is to be reference \cite{BanksFischer} does not evade the paradox. On the other hand, they do not refer to reference \cite{ilgin-yang-inside-old} that only postpones the problem to trans-Planckian physics.


ER~=~EPR.


Fuzzball Complementarity.


Papadodimas-Raju Proposal. Major criticism against this approach is that its state dependence violates quantum mechanics \cite{Almheiri2013}. This is because in this approach the interior of black hole is described by a subsystem of early radiation where the map that relates the two depends on the initial state of the black hole \cite{Almheiri2013}.


% Extreme Cosmic Censorship. This idea is not referred to in the AMPSS' paper \cite{Almheiri2013}. However Donald Marolf\ip{Marolf, Donald} and Joseph Polchinski's\ip{Polchinski, Joseph} article \cite{MarolfPolchinski}



Others. AMPSS rule out remnants by using AdS/CFT correspondence\ic{AdS/CFT correspondence}.





Finally, AMPSS express \cite{Almheiri2013} what their criticisms to various resolution attempts is ``the inconsistency of proposals allowing the release of energy by the black hole to be physically separated from the escape of information.'' Readers may be interested in \cite{ilgin-yang-energy-info} that puts emphasis on the physical nature of quantum information.

==> content/img/compl.tex <==
\begin{tikzpicture}[scale = 1, thick]
  \shade[ball color=black!20] (0,0) circle (1);
  \node[label=Outside obs., name=o] at (-4,0) {$\bullet$};
  \node[label=Ingoing obs., name=i] at ( 3,3) {$\bullet$};
  \draw[thin,postaction={decorate, decoration={markings, mark=between positions 0.1 and 1 step 0.1 with {\arrow{stealth}}}}] (3,3) -- (0,0);
  \node at (0,0) {$\star$};
\end{tikzpicture}

==> pgflibraryam.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter

% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{133}\def\@pgfornamentY{48}%  2
\fi%
}%
% appels des motifs 
\def\pgf@@ornament#1{%
\begingroup
\def\i{\pgfusepath{clip}}
\let\o\pgfpathclose
\let\s\pgfusepathqfillstroke
\def\p ##1##2{\pgfqpoint{##1bp}{##2bp}}
\def\m ##1 ##2 {\pgfpathmoveto{\p{##1}{##2}}}
\def\l ##1 ##2 {\pgfpathlineto{\p{##1}{##2}}}
\def\r ##1 ##2 ##3 ##4 {\pgfpathrectangle{\p{##1}{##2}}{\p{##3}{##4}}}
\def\c ##1 ##2 ##3 ##4 ##5 ##6 {%
\pgfpathcurveto{\p{##1}{##2}}{\p{##3}{##4}}{\p{##5}{##6}}}%
\@@input am#1.pgf 
%\@nameuse{pgf@@am@#1}%
\endgroup}%
\makeatother
\endinput   

==> pgflibraryvectorian.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter
% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{134}\def\@pgfornamentY{48}%  2
\or\def\@pgfornamentX{130}\def\@pgfornamentY{65}%  3
\or\def\@pgfornamentX{133}\def\@pgfornamentY{133}% 4
\or\def\@pgfornamentX{129}\def\@pgfornamentY{146}% 5
\or\def\@pgfornamentX{134}\def\@pgfornamentY{148}% 6
\or\def\@pgfornamentX{136}\def\@pgfornamentY{135}% 7
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 8
\or\def\@pgfornamentX{79}\def\@pgfornamentY{105}% 9
\or\def\@pgfornamentX{80}\def\@pgfornamentY{99}%  10
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  11
\or\def\@pgfornamentX{136}\def\@pgfornamentY{136}% 12
\or\def\@pgfornamentX{136}\def\@pgfornamentY{236}% 13
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  14
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  15
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  16
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  17
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  18
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  19
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  20
\or\def\@pgfornamentX{70}\def\@pgfornamentY{58}%  21
\or\def\@pgfornamentX{34}\def\@pgfornamentY{61}%  22
\or\def\@pgfornamentX{68}\def\@pgfornamentY{55}%  23
\or\def\@pgfornamentX{79}\def\@pgfornamentY{76}%  24
\or\def\@pgfornamentX{80}\def\@pgfornamentY{88}%  25
\or\def\@pgfornamentX{59}\def\@pgfornamentY{120}% 26
\or\def\@pgfornamentX{101}\def\@pgfornamentY{98}%  27
\or\def\@pgfornamentX{52}\def\@pgfornamentY{102}% 28
\or\def\@pgfornamentX{65}\def\@pgfornamentY{65}%  29
\or\def\@pgfornamentX{63}\def\@pgfornamentY{64}%  30
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  31
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  32
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  33
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  34
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  35
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  36
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 37
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 38
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 39
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 40
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 41
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 42
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  43
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  44
\or\def\@pgfornamentX{385}\def\@pgfornamentY{64}%  45
\or\def\@pgfornamentX{453}\def\@pgfornamentY{97}%  46
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  47
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  48
\or\def\@pgfornamentX{163}\def\@pgfornamentY{61}%  49
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 50
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 51
\or\def\@pgfornamentX{248}\def\@pgfornamentY{197}% 52
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 53
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 54
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 55
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 56
\or\def\@pgfornamentX{207}\def\@pgfornamentY{103}% 57
\or\def\@pgfornamentX{228}\def\@pgfornamentY{116}% 58
\or\def\@pgfornamentX{204}\def\@pgfornamentY{102}% 59
\or\def\@pgfornamentX{451}\def\@pgfornamentY{189}% 60
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 61
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 62
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 63
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 64
\or\def\@pgfornamentX{132}\def\@pgfornamentY{166}% 65
\or\def\@pgfornamentX{177}\def\@pgfornamentY{175}% 66
\or\def\@pgfornamentX{80}\def\@pgfornamentY{155}% 67
\or\def\@pgfornamentX{361}\def\@pgfornamentY{154}% 68
\or\def\@pgfornamentX{448}\def\@pgfornamentY{227}% 69
\or\def\@pgfornamentX{226}\def\@pgfornamentY{79}%  70
\or\def\@pgfornamentX{443}\def\@pgfornamentY{81}%  71
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  72
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  73
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  74
\or\def\@pgfornamentX{373}\def\@pgfornamentY{120}% 75
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  76
\or\def\@pgfornamentX{207}\def\@pgfornamentY{89}%  77
\or\def\@pgfornamentX{207}\def\@pgfornamentY{132}% 78
\or\def\@pgfornamentX{249}\def\@pgfornamentY{122}% 79
\or\def\@pgfornamentX{454}\def\@pgfornamentY{31}%  80
\or\def\@pgfornamentX{176}\def\@pgfornamentY{45}%  81
\or\def\@pgfornamentX{454}\def\@pgfornamentY{24}%  82
\or\def\@pgfornamentX{449}\def\@pgfornamentY{20}%  83
\or\def\@pgfornamentX{290}\def\@pgfornamentY{57}%  84
\or\def\@pgfornamentX{453}\def\@pgfornamentY{22}%  85
\or\def\@pgfornamentX{454}\def\@pgfornamentY{17}%  86
\or\def\@pgfornamentX{360}\def\@pgfornamentY{44}%  87
\or\def\@pgfornamentX{454}\def\@pgfornamentY{15}%  88
\or\def\@pgfornamentX{454}\def\@pgfornamentY{10}%  89
\fi%
}%
\makeatother
\endinput
